The FAST Galactic Plane Pulsar Snapshot survey: VIII. 116 binary pulsars

Finding pulsars in binaries are important for measurements of the masses of neutron stars, for tests of gravity theories, and for studies of star evolution. We are carrying out the Galactic Plane Pulsar Snapshot survey (GPPS) by using the the Five-hundred-meter Aperture Spherical radio Telescope (FAST). Here we present the Keplerian parameters for 116 newly discovered pulsars in the FAST GPPS survey, and obtain timing solutions for 29 pulsars. Companions of these pulsars are He white dwarfs, CO/ONe white dwarfs, neutron stars, main sequence stars and ultra light objects or even planets. Our observations uncover eclipses of 8 binary systems. The optical counterpart for the companion of PSR J1908+1036 is identified. The Post-Keplerian parameter $\dot{\omega}$ for the double neutron star systems PSR J0528+3529 and J1844-0128 have been measured, with which the total masses of the binary systems are determined.

==> table_Pdot.tex <==
\begin{table*}
  \centering
  \caption{Kinematic corrections of $\dot{P}$ and relavant parameters.}
  \label{tab:Pdot}
  \small
  %\footnotesize
  %\scriptsize
  \tabcolsep 1.2mm
  %\begin{rotatetable}

\begin{tabular}{crrrrrrrr}
\hline\hline
Pulsar & $\mu_T$       & $\dot{P}$     & $\dot{P_S}$  & $\dot{P_G}$ & $\dot{P_I}$ & $B_{\rm surf,c}$ & $\tau_c$ & $\dot{E_c}$ \\
       &($\rm mas~yr^{-1}$)&($10^{-21}s~s^{-1}$) & ($10^{-21}s~s^{-1}$) & ($10^{-21}s~s^{-1}$)& ($10^{-21}s~s^{-1}$) & ($10^8$Gs)    & (Gyr)    & ($10^{33} \rm erg~s^{-1}$) \\
(1)    & (2)           &(3)            & (4)          & (5)        & (6)         & (7)           & (8)      & (9)         \\
\hline
%\multicolumn{5}{c}{Observations} \\
%\hline
J1857+0642 & 5.9      &   4.69 & 0.30  &   0.03 &   4.36 &  1.26 & 12.80 & 3.91  \\
J1903+0839 & 5.0      &   4.67 & 1.49  &  -1.78 &   4.96 &  1.53 & 14.74 & 1.98  \\
J1904+0553 & 8.3      &  12.75 & 3.65  &  -0.94 &  10.04 &  2.25 &  7.72 & 3.36  \\
J1908+1036 &12.0      &  15.73 & 2.51  &  -0.03 &  13.25 &  3.81 & 12.75 & 0.43  \\
J1911+1253 & -      &  43.30 & -   &  -1.78 &  45.08 & 11.21 &  9.55 & 0.09  \\
J1916+0740 & -      &  20.00 & -   & -10.51 &  30.51 &  5.92 &  5.81 & 0.85  \\
J1917+1259 & -      &   6.54 & -   &  -1.16 &   7.70 &  2.11 & 11.56 & 1.70  \\
J1930+1403 & -      &   0.82 & -   &  -1.24 &   2.05 &  0.82 & 24.68 & 2.46  \\
J1947+2011 & -      &  23.17 & -   &  -3.10 &  26.27 &  4.69 &  4.92 & 1.90  \\
J1952+2837 & -      & 211.47 & -   & -13.06 & 224.53 & 20.36 &  1.27 & 1.52  \\
\hline

\end{tabular}

\tablenotes{
\item
Notes: $\mu_T$: total proper motion, $\dot{P_S}$: Shklovskii effect,
$\dot{P_G}$: Galactic acceleration, $\dot{P_I}$: intrinsic period derivative, 
$B_{\rm surf,c}$: corrected surface magnetic field, $\tau_c$: corrected age,
$\dot{E_c}$: corrected energy loss rate.
 }
%\end{rotatetable}
\end{table*}



==> table_PossiBinary.tex <==
\begin{deluxetable}{cccrrc}
\tablewidth{8pt}
\tablecaption{55 possible binary systems in FAST-GPPS. \label{tab:possiB}}
%\tabletypesize{\small}
%\colnumbers
\tabcolsep 0.5mm
\renewcommand{\arraystretch}{0.75}

\tablehead{\colhead{Pulsar} & \colhead{ $\alpha$} & \colhead{$\delta$} & \colhead{DM} & \colhead{$P$} & \colhead{Note}  \\ 
\colhead{} & \colhead{(h:m:s)} & \colhead{(d:m:s)} & \colhead{(cm$^{-3}$pc)} & \colhead{(ms)}  & \colhead{} } 

%% All data must appear between the \startdata and \enddata commands
\startdata
J0641+0448g & 06:41:33.3 & +04:48:37 & 155.1 & 25.672 & g0670 \\
J1814+0045g & 18:14:10.4 & +00:45:15 & 124.0 &  2.309 & g0549 \\
J1821+0044g & 18:21:31.7 & +00:44:23 & 126.9 &  2.713 & g0591 \\
J1828+0218g & 18:28:55.8 & +02:18:19 & 140.8 &  2.971 & g0686 \\
%J1829-0235g & 18:29:35.0 & -02:35:32 & 103.3 &  7.428 & g0599 \\
J1831+0204g & 18:31:19.8 & +02:04:58 & 115.2 &  2.079 & g0681 \\
J1832+0113g & 18:32:49.0 & +01:13:36 &  81.8 &  6.345 & g0665 \\
J1833-0048g & 18:33:53.0 & -00:46:00 &  81.4 &  2.954 & g0365, posi \\
J1834+0143g & 18:34:30.6 & +01:43:47 & 201.8 &  4.639 & g0647 \\
J1835-0011g & 18:35:47.8 & -00:11:52 &  36.2 &  3.230 & g0221 \\
J1835+0158g & 18:35:22.0 & +01:58:22 & 181.5 &  3.320 & g0636 \\
J1836+0117g & 18:36:11.7 & +01:17:46 & 178.0 &  3.812 & g0592 \\
J1837-0048g & 18:37:35.9 & -00:48:18 & 195.5 &  2.730 & g0326 \\
J1837+0528g & 18:37:40.5 & +05:28:29 & 120.8 &  6.260 & g0204 \\ 
J1838-0156g & 18:38:06.8 & -01:56:35 & 163.4 &  5.510 & g0267 \\ 
J1841-0123g & 18:41:08.6 & -01:23:52 & 308.2 &  3.790 & g0356 \\
J1844+0455g & 18:44:56.1 & +04:55:19 & 241.4 &  4.700 & g0598 \\
J1845+0104g & 18:45:50.4 & +01:04:39 &  95.0 &  6.714 & g0224 \\
J1846+0507g & 18:46:50.5 & +05:07:00 & 101.6 &  3.072 & g0614 \\
J1847+0342g & 18:47:30.6 & +03:42:36 &  81.1 &  4.289 & g0431 \\
J1855-0221g & 18:55:56.3 & -02:21:29 & 223.4 &  2.766 & g0533 \\
J1856+1000g & 18:56:30.3 & +10:00:23 & 202.1 &  4.870 & g0331 \\
J1857-0026g & 18:57:01.8 & -00:26:16 & 312.7 & 22.347 & g0454 \\
%J1857-0230g & 18:57:20.5 & -02:30:36 & 134.5 & 35.154 & g0577 \\
J1902+0011g & 19:02:40.2 & +00:11:05 & 248.5 &  5.928 & g0442 \\
J1904+0056g & 19:04:58.3 & +00:56:01 &  51.4 &  5.851 & g0441 \\
J1907+0009g & 19:07:21.5 & +00:09:51 &  83.0 &  2.375 & g0588 \\
J1907+0029g & 19:07:23.4 & +00:29:11 & 120.4 & 63.641 & g0573 \\
J1907+0052g & 19:07:57.5 & +00:52:00 & 162.9 &  2.921 & g0600 \\
J1908+0029g & 19:08:30.4 & +00:29:53 & 165.3 &  3.416 & g0633 \\
J1908+0949g & 19:08:07.8 & +09:49:53 & 220.1 &  9.049 & g0128 \\
J1910+0423g & 19:10:10.3 & +04:23:01 & 339.9 & 93.243 & g0432 \\
J1915+0601g & 19:15:56.2 & +06:01:30 & 151.8 &  4.011 & g0683 \\
J1915+0720g & 19:15:35.3 & +07:20:45 & 122.1 &  5.690 & g0413 \\
J1917+0923g & 19:17:45.4 & +09:23:46 & 297.8 &  4.710 & g0261 \\
J1917+1556g & 19:17:19.2 & +15:56:44 &  72.0 &  2.924 & g0471 \\
J1920+0129g & 19:20:37.6 & +01:29:35 & 104.1 &  3.580 & g0230 \\
J1921+1632g & 19:21:32.9 & +16:32:01 & 279.5 & 58.482 & g0550 \\
J1921+1652g & 19:21:34.0 & +16:52:20 & 124.1 &  3.680 & g0336 \\
J1924+1201g & 19:24:08.3 & +12:01:07 &  99.2 &  3.176 & g0461 \\
J1924+2110g & 19:24:10.1 & +21:10:17 &  93.4 &  5.037 & g0684 \\
J1929+1259g & 19:29:50.3 & +12:59:22 &  90.9 &  2.850 & g0345 \\
J1929+2355g & 19:29:44.8 & +23:55:07 & 206.8 &  4.790 & g0239 \\
J1931+2333g & 19:31:04.2 & +23:33:26 &  58.3 &  3.860 & g0675 \\
J1940+2102g & 19:40:13.6 & +21:02:08 &  76.2 & 30.051 & g0564 \\
J1942+2029g & 19:42:26.4 & +20:29:18 & 139.3 & 44.562 & g0660 \\
J1943+2847g & 19:43:36.5 & +28:47:23 & 191.6 &  6.296 & g0416 \\
J1946+2433g & 19:46:52.9 & +24:33:18 & 275.4 &  8.568 & g0366 \\
J1951+2352g & 19:51:21.8 & +23:52:13 & 259.2 & 48.394 & g0543 \\
J1951+2528g & 19:51:27.0 & +25:28:43 & 205.1 &  2.310 & g0210 \\
J1954+2833g & 19:54:11.3 & +28:33:44 &  37.0 & 27.210 & g0213 \\
J1955+3114g & 19:55:57.3 & +31:14:24 & 117.2 &  3.357 & g0692 \\
J1957+2711g & 19:57:35.8 & +27:11:24 & 210.4 & 23.374 & g0562 \\
J2000+3157g & 20:00:03.4 & +31:57:38 & 270.0 &  3.499 & g0590 \\
J2007+3343g & 20:07:53.0 & +33:43:53 & 217.2 &  2.681 & g0604 \\
J2032+4055g & 20:32:38.3 & +40:55:12 & 373.3 & 48.739 & g0623 \\
J2042+4353g & 20:42:53.2 & +43:53:41 & 292.6 & 16.016 & g0641 \\
\enddata

%\tablecomments{}

\end{deluxetable}

==> table_PostKep.tex <==
\begin{table*}
  \centering
  \caption{Expected Post-Keplerian parameters of 5 binary pulsars.}
  \label{tab:PostKep}
  \small
  %\footnotesize
  %\scriptsize
  \tabcolsep 0.5mm
  \renewcommand{\arraystretch}{0.7}
  %\begin{rotatetable}

\begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}
\hline\hline
%\multicolumn{4}{c}{Observation, assumption and measured quantities} \\
%\hline
Pulsar       & \multicolumn{3}{c}{$\gamma$} & \multicolumn{3}{c}{$\dot{\omega}$} & \multicolumn{3}{c}{$\dot{P_b}$} & \multicolumn{3}{c}{$\dot{x}$} & \multicolumn{3}{c}{$h_3$}       \\

             & \multicolumn{3}{c}{($\mu s$)}& \multicolumn{3}{c}{($^\circ/yr$)}   & \multicolumn{3}{c}{(s/s)}       & \multicolumn{3}{c}{(ls/s)}    & \multicolumn{3}{c}{($\mu s$)}   \\
%(1)          &(2)      & (3)     &  (4)         &  (5)      & (6)       &(7)      & (8)       \\
 $i=$        & 90$^\circ$ & 60$^\circ$ & 45$^\circ$ & 90$^\circ$ & 60$^\circ$ & 45$^\circ$ & 90$^\circ$ & 60$^\circ$ & 45$^\circ$ & 90$^\circ$ & 60$^\circ$ & 45$^\circ$ & 90$^\circ$ & 60$^\circ$ & 45$^\circ$  \\
(1)          &(2)      & (3)     &  (4)         &  (5)      & (6)       &(7)      & (8)    & (9)  & (10) & (11) & (12) & (13) & (14) & (15) & (16) \\
\hline
%\multicolumn{5}{c}{Observations} \\
%\hline
J0528+3529  & 5646  & 6994      & 9563    & 6.61e-3 & 7.08e-3 & 7.97e-3 & -7.1e-16 & -8.5e-16 & -1.1e-15 & -1.3e-15 & -1.5e-15 & -2.0e-15 & 5.66 & 1.35 & 0.69   \\
%J0622+0339  & 2.18e-2 & 2.57e-2 & 3.24e-2 & 6.06e-3 & 6.12e-3 & 6.24e-3 & -8.7e-17 & -1.0e-16 & -1.3e-16 & -3.0e-17 & -3.5e-17 & -4.3e-17 & 0.72 & 0.16 & 0.07   \\
%J1840+0012  & 1.77e-2 & 2.09e-2 & 2.64e-2 & 1.67    & 1.68    & 1.72    & -2.4e-14 & -2.8e-14 & -3.5e-14 & -2.6e-14 & -3.1e-14 & -3.8e-14 & 0.73 & 0.16 & 0.08   \\
%J1844+0028  & 4.44e-2 & 5.21e-2 & 6.57e-2 & 2.28e-1 & 2.30e-1 & 2.34e-1 & -3.1e-15 & -3.5e-15 & -4.4e-15 & -2.0e-15 & -2.3e-15 & -2.9e-15 & 0.66 & 0.15 & 0.07    \\
%J1845+0201  & 4.17e-2 & 4.94e-2 & 6.29e-2 & 1.64e-2 & 1.67e-2 & 1.71e-2 & -3.2e-16 & -3.7e-16 & -4.6e-16 & -1.8e-16 & -2.1e-16 & -2.6e-16 & 1.01 & 0.23 & 0.11    \\
%J1857+0642  & 3.15e-2 & 3.77e-2 & 4.90e-2 & 1.18e-2 & 1.22e-2 & 1.27e-2 & -3.7e-16 & -4.3e-16 & -5.4e-16 & -3.2e-16 & -3.8e-16 & -4.7e-16 & 1.78 & 0.41 & 0.19    \\
%J1903+0839  & 2.93e-3 & 3.44e-3 & 4.32e-3 & 1.78    & 1.80    & 1.83    & -2.1e-14 & -2.4e-14 & -3.0e-14 & -1.8e-14 & -2.1e-14 & -2.6e-14 & 0.57 & 0.13 & 0.06    \\
%J1904+0553  & 7.24e-3 & 8.51e-3 & 1.07e-2 & 1.21e-1 & 1.22e-1 & 1.24e-1 & -1.7e-15 & -1.9e-15 & -2.4e-15 & -1.0e-15 & -1.2e-15 & -1.4e-15 & 0.69 & 0.15 & 0.07    \\
%J1905+0649  & 1.97e-1 & 2.43e-1 & 3.30e-1 & 2.02e-1 & 2.15e-1 & 2.38e-1 & -1.2e-14 & -1.5e-14 & -1.9e-14 & -4.0e-14 & -4.7e-14 & -6.1e-14 & 4.70 & 1.11 & 0.55    \\
%J1908+1036  & 6.21e-3 & 7.59e-3 & 1.02e-2 & 3.31e-2 & 3.47e-2 & 3.78e-2 & -1.8e-15 & -2.1e-15 & -2.7e-15 & -3.4e-15 & -4.0e-15 & -5.1e-15 & 3.78 & 0.88 & 0.44    \\
J1911+1253  & 53.27   & 64.82   & 86.30   & 5.15e-3 & 5.38e-3 & 5.78e-3 & -2.4e-16 & -2.9e-16 & -3.7e-16 & -2.8e-16 & -3.3e-16 & -4.2e-16 & 3.15 & 0.73 & 0.35    \\        
%J1912+1416  & 5.03e-3 & 5.90e-3 & 7.40e-3 & 2.64    & 2.66    & 2.70    & -2.9e-14 & -3.4e-14 & -4.2e-14 & -2.6e-14 & -3.0e-14 & -3.8e-14 & 0.54 & 0.12 & 0.06    \\
%J1916+0740  & 5.65e-2 & 6.66e-2 & 8.43e-2 & 2.93e-3 & 2.97e-3 & 3.03e-3 & -4.7e-17 & -5.5e-17 & -6.7e-17 & -1.5e-17 & -1.8e-17 & -2.2e-17 & 0.81 & 0.18 & 0.08    \\
%J1917+0615  & 8.86e-2 & 1.05e-1 & 1.33e-1 & 2.06e-2 & 2.08e-2 & 2.13e-2 & -3.5e-16 & -4.0e-16 & -5.0e-16 & -1.8e-16 & -2.1e-16 & -2.6e-16 & 0.86 & 0.19 & 0.09    \\
%J1917+1259  & 2.02e-1 & 2.43e-1 & 3.18e-1 & 4.16e-2 & 4.28e-2 & 4.49e-2 & -1.4e-15 & -1.7e-15 & -2.1e-15 & -1.7e-15 & -2.0e-15 & -2.6e-15 & 1.99 & 0.46 & 0.22    \\
%J1918+0621  & 6.15e-2 & 7.22e-2 & 9.10e-2 & 2.15e-2 & 2.17e-2 & 2.21e-2 & -2.9e-16 & -3.4e-16 & -4.1e-16 & -1.2e-16 & -1.4e-16 & -1.7e-16 & 0.66 & 0.15 & 0.07    \\
%J1924+1342  & 4.28e-2 & 5.00e-2 & 6.25e-2 & 3.10e-2 & 3.13e-2 & 3.16e-2 & -2.9e-16 & -3.3e-16 & -4.1e-16 & -8.8e-17 & -1.0e-16 & -1.3e-16 & 0.45 & 0.10 & 0.05    \\
%J1930+1403  & 5.30e-2 & 6.29e-2 & 8.04e-2 & 1.54e-2 & 1.57e-2 & 1.61e-2 & -3.3e-16 & -3.8e-16 & -4.8e-16 & -2.0e-16 & -2.4e-16 & -3.0e-16 & 1.13 & 0.25 & 0.12    \\
%J1932+2121  & 9.24e-3 & 1.08e-2 & 1.36e-2 & 16.96   & 17.11   & 17.35   & -2.0e-13 & -2.3e-13 & -2.8e-13 & -2.6e-13 & -3.1e-13 & -3.8e-13 & 0.57 & 0.13 & 0.06    \\
%J1936+2035  & 3.91e-1 & 4.82e-1 & 6.54e-1 & 3.15e-1 & 3.34e-1 & 3.71e-1 & -1.9e-14 & -2.3e-14 & -3.0e-14 & -6.9e-14 & -8.2e-14 & -1.1e-13 & 4.79 & 1.13 & 0.57    \\
J1938+2302  &  8.95   & 11.01   & 14.90   & 9.65e-4 & 1.02e-3 & 1.13e-3 & -5.8e-17 & -6.9e-17 & -8.9e-17 & -6.2e-17 & -7.4e-17 & -9.5e-17 & 4.54 & 1.07 & 0.53    \\
%J1943+2206
J1946+0904  &  1.35   &  1.61   &  2.08   & 1.39e-2 & 1.42e-2 & 1.48e-2 & -3.8e-16 & -4.5e-16 & -5.6e-16 & -3.0e-16 & -3.5e-16 & -4.4e-16 & 1.52 & 0.35 & 0.16   \\
J1947+2011  &  1.19   &  1.43   &  1.84   & 1.79e-4 & 1.82e-4 & 1.89e-4 & -4.6e-18 & -5.4e-18 & -6.7e-18 & -1.4e-18 & -1.6e-18 & -2.1e-18 & 1.40 & 0.32 & 0.15    \\
%J1952+2837  & 1.37e-2 & 1.63e-2 & 2.09e-2 & 3.46e-1 & 3.52e-1 & 3.64e-1 & -8.2e-15 & -9.5e-15 & -1.2e-14 & -1.0e-14 & -1.2e-14 & -1.5e-14 & 1.26 & 0.29 & 0.13    \\
%J2018+3518  & 4.86e-1 & 6.00e-1 & 8.15e-1 & 4.75e-2 & 5.05e-2 & 5.63e-2 & -3.0e-15 & -3.6e-15 & -4.6e-15 & -7.5e-15 & -8.9e-15 & -1.2e-14 & 4.99 & 1.18 & 0.59   \\

\hline
\end{tabular}

%\tablenotes{
%\item
Notes: $i$: inclination angle, $\gamma$: magnitude of Einstein delay,
$\dot{\omega}$: rate of periastron advance, $\dot{P_b}$: rate of
orbital decay, $\dot{x}$: rate of axis decay, $h_3$: orthometric
amplitude. Orthometric ratio $\zeta$=1.0, 0.58 and 0.41 for
inclination angles of 90$^\circ$, 60$^\circ$ and 45$^\circ$. The
parameters are estimated by assuming $m_p=1.35M_\odot$.
%}
%\end{rotatetable}
\end{table*}



==> table_optical.tex <==
\begin{table*}
  \centering
  \caption{Limits of optical counterparts of 16 WD binaries from WD cooling models.}
  \label{tab:opt}
  \small
  %\footnotesize
  %\scriptsize
  \tabcolsep 1.2mm
  \renewcommand{\arraystretch}{0.7}
  %\begin{rotatetable}

\begin{tabular}{cccccccccrr}
\hline\hline
Pulsar & $E$  & \multicolumn{5}{c}{$M_l$}  & $m_{c,m} (M_{\odot})$ & Cons.Band  & $T_{\rm eff} (K)$ & $\rm Age (Gyr)$  \\
       &      &  g & r & i & z & y         &                    &            &                 &                  \\
 (1)   & (2)  & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10)  & (11) \\
\hline
%\multicolumn{5}{c}{Observations} \\
%\hline
%J0528+3529 & 0.677 & 21.010 & 21.520 & 21.856 & 21.343 & 20.638 & 1.3 & y & $<$2250  & $>$5.56 \\
J0622+0339 & 0.696 & 20.946 & 21.473 & 21.821 & 21.316 & 20.617 & 0.2 &   &          &         \\
%J1840+0012 & 1.841 & 17.070 & 18.629 & 19.716 & 19.697 & 19.327 & 0.2 & g & $<$3000  & $>$4.62 \\
J1844+0028 & 1.472 & 18.320 & 19.546 & 20.395 & 20.219 & 19.743 & 0.2 & g & $<$2000  & $>$9.85 \\
J1845+0201 & 1.813 & 17.163 & 18.697 & 19.767 & 19.736 & 19.358 & 0.2 & g & $<$3000  & $>$4.62  \\
J1857+0642 & 2.784 & 13.879 & 16.287 & 17.983 & 18.363 & 18.265 & 0.4 & g & $<$6000  & $>$1.47 \\
%J1903+0839 & 2.044 & 16.383 & 18.125 & 19.343 & 19.410 & 19.099 & 0.2 & g & $<$3500  & $>$3.55 \\
J1904+0553 & 2.430 & 15.078 & 17.167 & 18.634 & 18.865 & 18.664 & 0.2 & g & $<$4500  & $>$2.13 \\
J1905+0649 & 2.129 & 16.095 & 17.914 & 19.187 & 19.289 & 19.003 & 1.2 & g & $<$6000  & $>$5.68 \\
%J1908+1036 & 0.668 & 21.038 & 21.541 & 21.872 & 21.355 & 20.647 & 0.9 & y & $<$1750  & $>$13.41 \\
J1911+1253 & 1.222 & 19.165 & 20.166 & 20.854 & 20.572 & 20.024 & 0.8 & g & $<$2250  & $>$13.61 \\
%J1912+1416 & 1.030 & 19.816 & 20.643 & 21.208 & 20.844 & 20.241 & 0.2 &   &          &          \\
J1916+0740 & 1.332 & 18.794 & 19.894 & 20.653 & 20.417 & 19.901 & 0.2 & g & $<$1750  & $>$11.66 \\
J1917+0615 & 1.170 & 19.340 & 20.294 & 20.949 & 20.645 & 20.082 & 0.2 &   &          &          \\
J1917+1259 & 1.761 & 17.342 & 18.829 & 19.864 & 19.811 & 19.418 & 0.5 & g & $<$3250  & $>$10.13 \\
J1918+0621 & 1.042 & 19.775 & 20.614 & 21.186 & 20.827 & 20.227 & 0.2 &   &          &          \\
J1924+1342 & 1.688 & 17.587 & 19.008 & 19.997 & 19.913 & 19.499 & 0.2 & g & $<$2500  & $>$6.95   \\
J1930+1403 & 1.547 & 18.066 & 19.360 & 20.257 & 20.113 & 19.659 & 0.3 & g & $<$2250  & $>$10.19 \\
%J1932+2121& 1.616 & 17.830 & 19.187 & 20.129 & 20.014 & 19.580 & 0.2 & g & $<$2250  & $>$8.35  \\
J1936+2035 & 1.770 & 17.309 & 18.804 & 19.846 & 19.797 & 19.407 & 1.2 & g & $<$5000  & $>$7.25  \\
%J1938+2302 & 1.326 & 18.813 & 19.908 & 20.663 & 20.425 & 19.907 & 1.1 & g & $<$3250  & $>$9.92  \\
%J1943+2206 &       &        &        &        &        &        &     &   &          &           \\
J1947+2011 & 0.520 & 21.539 & 21.908 & 22.143 & 21.564 & 20.814 & 0.3 & y & $<$1500  & $>$15.41 \\
%J1952+2837 & 1.227 & 19.148 & 20.153 & 20.845 & 20.565 & 20.018 & 0.3 & g & $<$1500  & $>$15.41 \\
J2018+3518 & 2.836 & 13.702 & 16.158 & 17.887 & 18.290 & 18.206 & 1.2 & g & $<$11000 & $>$2.35  \\
\hline

\end{tabular}

%\tablenotes{
%\item
Notes: $E$: reddening from Bayestar17 model, $M_l$: magnitude limit at
each of the grizy band, $m_{c,m}$: mass of WD companion in cooling
models, Cons. Band: band of grizy employed to constrain $T_{\rm eff}$
and $\rm Age$, $T_{\rm eff}$: effctive temperature, $\rm Age$: WD age.
%}
%\end{rotatetable}
\end{table*}


